Lifted Relational Algebra with Recursion and Connections to Modal Logic

We propose a new formalism for specifying and reasoning about problems that involve heterogeneous "pieces of information" -- large collections of data, decision procedures of any kind and complexity and connections between them. The essence of our proposal is to lift Codd's relational algebra from operations on relational tables to operations on classes of structures (with recursion), and to add a direction of information propagation. We observe the presence of information propagation in several formalisms for efficient reasoning and use it to express unary negation and operations used in graph databases. We carefully analyze several reasoning tasks and establish a precise connection between a generalized query evaluation and temporal logic model checking. Our development allows us to reveal a general correspondence between classical and modal logics and may shed a new light on the good computational properties of modal logics and related formalisms.

==> Introduction.tex <==






	
\ignore{

\begin{quote}	
	{\it ``There is a point where in the mystery of\\
		existence contradictions meet;\\
		where movement is not all movement\\
		and stillness is not all stillness;\\
		where the idea and the form,\\
		the within and the without, are united;\\
		where infinite becomes finite,\\
		yet not losing its infinity.''\\
		Rabindranath Tagore}
	
\end{quote}

}


\begin{quote}	\begin{small}
	{\it ``There is a point where in the mystery of
		existence contradictions meet;
		where movement is not all movement
		and stillness is not all stillness...
		where the idea and the form,
		the within and the without, are united;
		where infinite becomes finite,
		yet not losing its infinity.''}
{\it ${\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ }	$ Rabindranath Tagore}
	\end{small}
	\end{quote}

	
\ignore{

design, semantics, query languages

data models, data structures, algorithms for data management

concurrency and recovery, distributed and parallel databases, cloud computing

model theory, logics, algebras, computational complexity

graph databases and (semantic) Web data

data mining, information extraction, search

data streams

data-centric (business) process management, workflows, web services

incompleteness, inconsistency, uncertainty in databases

data and knowledge integration and exchange, data provenance, views and data warehouses, metadata management

domain-specific databases (multi-media, scientific, spatial, temporal, text)

deductive databases

data privacy and security
}
	

%{\tt This introduction is from a different paper. It will be replaced of course, but I am keeping it here for now 
%	to show where it is all going.}





In 1970	Edgar (Ted) F. Codd introduced a relational data model
and two query languages:  relational calculus and relational algebra.
Relational calculus is what we usually call FO logic.
The key contribution of Codd was to associate with a declarative specification language (FO logic),
	a procedural counterpart which is the relational algebra, that later was implemented by smart engineers  and  became
	a multi-billion dollar industry of relational database
	management systems (RDBMS). 


%amount of data, the radical shift in the amount of data, in the way that scientists distribute, 
%store, and aggregate this data, precipitates new challenges for knowledge representation

%scallability



A significant change has happened in the past decade.  
While, at the low level, everything data-related boils down to  SQL queries,
{\em interactions  between ``larger'', combinatorially harder, pieces became increasingly important.}
Such ``larger pieces'' are business enterprises, 
 web services, software, solvers in the world of declarative problem solving, {\tt collections of learned data, potentially with numeric ranking assigned
 	 } etc.
The emergence of large-scale interactions poses  significant challenges to 
 database researchers. Among those challenges,  the most urgent is  {\em scallability of proposed approaches to data management}.
%reflects the radical shift in the amount of data and its nature. 
%Among many directions in development of data management, the most urgent is its {\em scallability}.
The importance of scallability is supported by the
 Moore's Law (1965), according to which the number of transistors in a dense
integrated circuit doubles approximately every two years. {\tt add citatoin}
Moore's prediction proved accurate for several decades:
capabilities of hardware has been growing exponentially, a fenomenon that have been partially responsible for the 
spectacular progress in technology for solving NP-hard problems, -- SAT, SMT, ILP. 

{\tt It is very likely that supercomputers (even quantum computers) will be a utility that is easily available.  
	 }

{\tt People already combine solvers \red{not only solvers, give examples}, but do it on a case-by-case basis,
	and no systematic approach exists}.
We expect  that, as hardware capabilities grow, people
	should be able to combine, as easily as relational tables in SQL queries,
	entities of a completely different magnitude:
	knowledge bases, ontologies,
		% e.g. representing the work of
	%	various enterprises, into complex business processes,
		{\em specifications}, e.g.  of combinatorial optimization and search problems, declarative and imperative 
pieces of software or web services.
%for solving new, more complex, problems.

       


\ignore{\tt
 	
 		Combinations of solvers (motivated by suitability of the corresponding modelling language to particular sub-problems)
 		is already a reality. Notable examples include Satisfiability Modulo Theory (SMT) solvers, ASP-CP combinations,
 		integrated modelling languages such as Comet in the CP community.
 		
 		
 	
 	CP
 	
 	http://www.imada.sdu.dk/~marco/Teaching/
 	
 	AY2011-2012/DM826/Slides/dm826-lec1.pdf
 	see the file saved
 	
 	Excellent examples!
 	
 	Hybrid Methods Hybrid Modelling
 	Strengths:
 	CP is excellent to explore highly constrained combinatorial spaces quickly
 	Math programming is particulary good at deriving lower bounds
 	LS is particualry good at derving upper bounds
 	How to combine them to get better “solvers”?
 	Exploiting OR algorithms for filtering
 	Exploiting LP (and SDP) relaxation into CP
 	
 	Integrated Modeling
 	
 	Models interact with solution process hence models in CP and IP are
 	different.
 	To integrate one needs:
 	to know both sides
 	to have available a modelling language that allow integration
 	(Comet)
 	There are typcially alternative ways to formulate a problem. Some may yield
 	faster solutions.
 	Typical procedure:
 	begin with a strightforward model to solve a small problem instance
 	alter and refine the model while scaling up the instances to maintain
 	tractability
 	13
 }
 
 
\ignore{ 
To be more concrete, let us think that each one of these  heterogeneous ``larger pieces'' is represented declaratively, e.g.,
 by Logic Programming rules, ILP equations, SMT theories, FO knowledge bases, etc.

The main challenge
is that the programs may be written in different languages (even legacy 
languages), and rely on different solving technologies, and business enterprises may look like ``black boxes'' from the outside.
	\blue{Interactions between business enterprises (back boxes) and web service compositions
		can also be modelled through compositions of classes of structures. }
	
	}
	




\ignore{\tt 
 algorithms for solving is the main and the most important direction. 
	
	Solutions have to jointly satisfy the combinatorial 
	optimisation solvers and the algebraic expression. 
	We have two papers on that, and are working on more. 
	There is a lot that needs to be done.
	
	
	
	
	One direction I am considering is to have those databases
	be learned from text documents (e.g. financial reports, election polls etc.).
	So, statistical learning needs to be involved. I have a student 
	working on a version of the algebra where weights (e.g. probabilities) 
	are assigned to structures and collections of structures. 
	
	}	
	
	

While  database queries, expressed using Codd's  relational calculus, can be viewed 
as   {\em relations definable with respect to a structure} (a database),
{declarative problem specifications} can be understood as  
{ \em axiomatizations of classes of structures}.
The two notions 	 (in italic)	are defined in two consecutive chapters in the classic textbook 
on mathematical logic \cite{Enderton}.

\noindent{\bf First Idea: Lifting Codd's Algebra}
Our first main idea is to lift  Codd's algebra from operations on relational tables to operations 
on {\em classes of structures} (which we call modules). Each module could be  a 
collection of databases, or a database that is not fully visible from the outside and thus is viewed as a 
collection of databases (since  unknown parts may have multiple interpretations). 
 A module can be given explicitly or implicitly, 
 e.g.  by a knowledge base,
 by an ontology, or by a constraint handling formalism such as 
 Answer Set Programming  (ASP), Integer Linear Programming (ILP), 
 Constraint programming (CP), Propositional Satisfiability (SAT), etc.
 It can even be ........ 
 
Later on, we will add information propagation to the algebra, which is our second main idea.



\begin{example}\label{ex:HC-2Col} {\tt say that a combinatorial problem is a class of structures\footnote{A module is a {\em set} of structures when the domain is fixed.}}
	{\rm  
		Let $M_{\rm HC}(V,X,Y)$ and $M_{\rm 2Col}(V,X,Z,T)$ be atomic modules ``computing'' a Hamiltonian Circuit, and a 2-colouring. They can do it in different ways.
		For example, $M_{\rm HC}$ can be an Answer Set Programming program, and $M_{\rm 2Col}$ be an imperative program or a human child with two pencils.  Here, $V$ is a relational variable of arity 1, $X,Y$ are relational variables of arity 2, and the first module decides if $Y$ forms a Hamiltonian Circuit (represented as a set of edges) in the graph given by vertex set $V$ and edge set $X$. Variable $X$ of the second module has arity 2, and variables $Z,T$ are unary; the module decides if unary relations $Z,T$ specify a proper 2-colouring of the graph with edge set $X$. The following algebraic expression determines a combination of 2-Colouring and Hamiltonian Circuit, that is whether or not there is a 2-colourable Hamiltonian Circuit.\footnote{We use $:=$ for ``is by definition''.}
		\begin{equation} \label{3-Col-HC}
		\begin{array}{l}
		M_{\rm 2Col-HC}( V,X,Z,T) \ :=\  \\
		%%  \hspace{-5mm}	\pi_{E_1,Col} (\sigma_{C_V\equiv E_2)} (M_{\rm HC}(E_1, C_V) \times 	M_{\rm 3Col}(E_2,Col)).
		\hspace{-5mm}	\pi_{V, X,Z,T} ((M_{\rm HC}(V, X, Y) \times 	M_{\rm 2Col}(V, Y,Z,T)). 	
		\end{array}
		\end{equation}
		%% Here,  the selection  operator requires the interpretations of $C_V$ in $M_{\rm HC}$ and of $E$ in $M_{\rm 3Col}$ to be the same.
		%% Thus, Hamiltonian Circuit gets coloured. 
		
	{\tt explain the operations: like in Codd's algebra, but applied on classes of structures}
		Projection ``keeps'' $V,X,Z,T$ and  hides   the interpretation of $Y$ in  $M_{\rm HC}$, since it is the same as $Y$'s in $M_{\rm 2Col}$.
	}
\end{example}





\begin{example}        \label{ex:LSP}   
	{\rm  	This modular system can be used by a company that provides logistics services 	(arguments of atomic modules are omitted).
		$$M_{LSP}:= \sigma_{B\equiv B'}(M_K \times M_{TSP}).$$
		It decides how to pack goods and
		deliver them.
		It solves two NP-complete tasks interactively, -- Multiple Knapsack (module $M_K$) and Travelling Salesman Problem (module $M_{TSP}$).
		The system takes orders from customers (items  to deliver, their profits, weights), and the capacity of trucks, decides how to pack  items in trucks, and for each truck, 
		solves a TSP problem. 
		The feedback ????????? $B'$ about solvability of TSP is sent back to $M_K$.
		%	Module $M_{TSP}$ takes a candidate solution from $M_K$, together with the graph of cities and routes with distances, allowable distance limit and destinations for each product. It computes the route for each truck. 
		%	The Knapsack problem is solved, 
		% e.g. using Integer Linear Programming (ILP), and TSP using Answer Set Programming (ASP), and they are 
		The two sub-problems, $M_K$ and $M_{TSP}$, are solved by different sub-divisions of the company (with their own business secrets) that cooperate towards the common goal. 
		%	The modules $M_K$ and $M_{TSP}$ are composed in sequence, with a feedback going from an output 
		%	of $M_{TSP}$ to an input of $M_K$.  
		A solution to the compound module, $M_{LSP}$, to be acceptable, must satisfy both sub-systems.
	}
\end{example}




Many practical examples use simple combinations of modules, where only conjunctions, disjunctions, perhaps with projections and selections, are used.
%The university timetabling example \cite{JOJN} and Examples \ref{ex:HC-2Col}, \ref{ex:LSP} are of this kind. 
But in other specifications, the use of a {\bf recursive construct} is essential. We may need to specify a recursive algorithm,
or the semantics of the satisfaction relation in a logic, which is given by an inductive definition.

\ignore{
Examples where a (declaratively specified) module 
calls itself recursively are much harder to come by.
We will however show two  natural applications. In the first one, 
combinatorial  search problems on graphs are solved using their tree decompositions. 
}


In the following example, recursion is used to specify an algorithm for solving a combinatorial search problem on graphs using  tree decompositions. 
\begin{example}{\rm 
In one of the applications we consider below, we need recursion to specify a Dynamic Programming algorithm on a tree decomposition of a graph.
The modules we use are $M_{\rm TD}$ that performs tree decomposition of each graph, and
 $M_{\rm 3Col}$ that performs 3-Colouring. 
The problem is represented~as \begin{small}
	$$M_{\rm TD} \land \mu Z. \Psi ( Z, M_{\rm TD},M_{\rm 3Col}  ),$$ 
\end{small}
\noindent where  $Z$ is a module variable over which recursive iteration is performed, the least fixed point expression
$\mu Z. \Psi ( Z, M_{\rm TD},M_{\rm 3Col}  ) $ specifies the dynamic programming algorithm.
Details will be explained in Example~\ref{Ex:TD}.\\
}


\end{example}

\begin{example} {\rm 
One can solve satisfiability problem for varous logics by axiomatizing the satisfaction relation for those logics and 
	then solving the satisfiability of the formulas given on the input  by running a universal solving engine, as is done 
	in e.g. \cite{Bart-IJCAI}.	
	 The satisfaction relation is inherently recursive. {\tt FO(LFP)= WF-DATALOG }}
\end{example}

\begin{example} {\rm 
		{\tt Pressburger arithmetic example }		\blue{TO DO}
	}
\end{example}

\begin{example} {\rm 
		{\tt FO-expression complexity example }		\blue{TO DO}
	}
\end{example}


\begin{example} {\rm 
		{\tt LTL example }		\blue{TO DO}
	}
\end{example}

\begin{example} {\rm 
In another application, we need recursion to specify an algorithm for solving quantified boolean formulas (QBFs).
The specification we obtain defines the semantics of QBFs. Similar ideas can be applied to defining the semantics 
of many other expressive logics.
}
\end{example}


\begin{example} {\rm 
		In this application, we specify the semantics of monadic second-order logic (MSO) of one successor 
		over strings. \blue{TO DO	}}
\end{example}




A significant break-through happened in the area of formal verification. Amir Pnueli received the Turing award in 1996
	for the introduction of temporal logic as a specification language for system behaviour . ...  Since then. the abstract notion of a dynamic system, plays an important role .... 
	... represents ongoing input-output 
	behaviour of a system.  

Problem solving often involves finding solutions for given inputs.
We observe that most combinatorial problems are of that form, many software programs and hardware devices are of that form. 
The Logistics Service Provider in Example  \ref{ex:LSP} has, e.g., customer requests
as an input, and routes and packing solutions as  outputs.
One can 
have e.g. edges of a graph on the input 
to formula  (\ref{3-Col-HC}), and colours on the output. 






\noindent{\bf Second  Idea: Adding Information Propagation} Our second idea is to add  
information flow to the algebra.     Modules with information propagation  become 
binary higher-order input-output relations or \\ {\em non-deterministic actions}.
Modules without information propagation become {\em propositions}.
Interpreting our algebra over a transition system
gives rise to a modal temporal logic. 


	
	
------------

	
	Funding solutions to the algebraic expressions can be done by advancing 
	the techniques developed in the SAT community, as well as those 
	developed in the verification community.



Thus, the algebra with information flow may be called ``a logic of hybrid MX tasks''.\footnote{An interesting version  is where only some inputs and outputs are specified, and some modules, even though {\em are known 
		to be binary}, do not have input-output assignments for their relational variables.
	In this case, we obtain a collection of transition systems, one for each possible assignment, and both sceptical (under all input-output assignments) and brave reasoning 
	(under some input-output assignment) can be studied. }


%{\em Model expansion is the dominant task of all constraint solving technologies.}


\here{give examples of modal logic expressions}



\here{ use techniques developed in temporal MC }


\here{ uniform solving process} 
-------------



\ignore{\here {The introduction abruptly moves from a general motivation to the definition of the algebra, which comes out of the blue and is actually repeated later on in the paper.}
}


\ignore{

Each atomic module can be given, e.g., by a set of constraints in a constraint formalism 
that has an associated solver, such as Answer Set Programming or 
Constraint Satisfaction Problem, it can be an agent or a business enterprise.  Satisfaction relation for each module is formalism-specific, 
e.g., it can be Stable Model semantics 
in case of ASP modules, and here it is abstractly represented by an interpretation that assigns
a class of structures to a module.
}

 
\subsubsection{Contributions}

{\red {an easy way to model data flow }

\footnote{ Here, we require a model-theoretic semantics, although various generalizations are possible.
}



----------------------------


Under the ``still''  or ``static'' view, the algebra is the same as Codd's relational 
algebra (with recursion added), but operations are applied to classes of structures 
instead of relational tables.
Under the ``dynamic'' view, when we indicate the direction of information flow, 
the same algebra is a modal temporal logic.

the lifted Codd's RA becomes a modal temporal logic when information propagation is added. 
Each state in the resulting dynamic system is a structure, or a set of ground atomic 
formulas, which is analogous to a state being determined by a set of atomic propositions in 
temporal logics such as LTL. CTL, $L\mu$.


-----------------------



We use the algebra for a high-level encoding of problem solving on graphs using Dynamic Programming on tree decompositions.
We also use it to specify an algorithm for solving quantified boolean formulas.



	We show that the well-known Propositional Dynamic Logic is a fragment of the algebra with information flow.
	
	We demonstrate a connection of our formalism to the situation calculus with the cognitive robotics language Golog.
	%is an axiomatic representation of a rich fragment of the algebra.








\ignore{
\subsubsection{Related Work}

Recently, there has been a lot of work on  {\em technology integration}. 
%both 	on the level of solvers and on the level of formalisms.
Examples include but are not limited to 
\cite{DBLP:journals/amai/MellarkodGZ08,DBLP:conf/lpnmr/BalducciniLS13,DBLP:conf/cpaior/0001KMO14,ASP-CP-combination,Picat}. %We do not attempt  a comprehensive survey, but we highlight some important issues.
Combined solving is perhaps most developed in the SMT community, where theory propagations are tightly interleaved with satisfiability solving
\cite{DBLP:journals/jacm/NieuwenhuisOT06,SMT}.
Declarative and imperative types of programming sometimes have to be combined for best results.

}




\section{Preliminaries} 

{\tt We assume familiarity with ..}

A {\em vocabulary} (denoted, e.g. $\tau,\sigma,\varepsilon,\nu$) is a finite sequence of non-logical  (predicate and function) symbols,
each with an associated arity.
A $\tau$-structure, e.g.
 $$\strA=(A;S_{1}^{\strA}, ...,S_{n}^{\strA}, f_{1}^{\strA},...,f_{m}^{\strA}, c_{1}^{\strA},...,c_{l}^{\strA})$$
  is a domain $A$ together with interpretations of predicate symbols, function and constants (0-ary functions) in $\tau$.
To simplify presentation,   we view functions as a particular kind of relations and consider relational structures only.
%Sometimes we have the need to talk about structures without specifying a particular vocabulary that structure interprets. 
%In those cases, we simply give a relational structure as a domain and a finite sequence of relations on that domain, e.g., $(D; R_1,\dots R_n)$. 
We use notations  $vocab(\strA)$, $vocab(\phi)$, $vocab(M)$ to denote 
vocabulary of structure $\strA$, formula $\phi$ and module $M$, respectively, and 
\red{we use ${\strB}|_{\sigma}$ to mean structure ${\strB}$ restricted to vocabulary $\sigma$.}
%We use $vocab(\phi)$, $vocab(M)$ to refer to the vocabulary of a formula and a module, respectively.
Symbol $:=$ means ``denotes'' or ``is by definition''.


There are several examples of connections between classical (``still'' or ``static'') and modal (``dynamic'') logics, and the notion of bisimulation 
plays an important role there. These are the so-called {\em model-theoretic characterization theorems}. For example,  
van Benthem shown that modal logic is a bisimulation-invariant fragment of first-order logic.
Janin and Walukiewicz proved that the modal $\mu$-calculus  $L\mu$ is the bisimulation-invariant 
fragment of monadic second-order logic MSO.
\cite{DBLP:conf/aiml/ZaidGJ14} studied a related notion of bisimulation safety introduced by van Benthem.
They introduced a new logic called Bisimulation Safe Fixed Point Logic (BSFP) that is more expressive than MSO.
The BSFP logic is a very elegant formalism that uses both unary and binary fixed points. 
We will discuss it in more detail and use this logic in the context of modular systems with information flow.
We investigate connections with other modal temporal logics. From the connection to BSFP logic, it follow that 
Propositional Dynamic Logic (PDL) is a fragment of  our algebra with information flow. 


We were quite surprised to notice that essentially the same 
constructions as in BSFP, but in axiomatic setting, appeared some 18 years earlier 
in the context of the situation calculus and GOLOG \cite{Levesque97-Golog,DTR}.
We discuss connections to the situation calculus in detail.

The duality of the ``static'' and ``dynamic'' views on modular systems opens new possibilities 
for developing  algorithms to answer questions about the ``static'' algebra.
For example, finding solutions 
to multi-language constraint problems can be done by solving Model Checking 
task for the modal temporal logic. This  implies that 
both SAT-based and symbolic model checking techniques can be used.


%	The MC-MX correspondence paves a way to  symbolic methods for solving modular systems. 










\ignore{

The Constraint Satisfaction Problem (CSP) in the traditional AI form is: \underline{Instance}: 
$ (V,D,C)$ where $V$ is a finite set of variables, $D$ is a set of {\em values} (also called domain),
$C$ is a finite set of {\em constraints} $\{C_1,\dots, C_n\}$. Each constraint is a pair $(\overline{x}_i,R_i)$,
where $\overline{x}_i$ is the {\em scope}, a list of variables of length $m_i$, and $R_i$ is a {\em $m_i$-ary relation} over $D$.
\underline{Question:} 
Is there $f : V \rightarrow D $ such that  $f(\overline{x}_i) \in R_i$ for all $i$? 
One can also search for such $f$.

A homomorphism  is a function $h : \strA \rightarrow \strB$ such that 
$\forall i [(a_1, \dots , a_{n_i}) \in R^{\strA}_i \Rightarrow (h(a_1), . . . , h(a_{n_i})) \in R^{\strB}_i ]$.

CSP in homomorphism form is: \underline{Instance}: Two $\tau$-structures, $\strA$ and $\strB$.
\underline{Question:} Is there a homomorphism  $h : \strA \rightarrow \strB$?
To relate to the AI form of CSP, 
	think of domain elements in $\strA$ as of variables.
	Tuples in relations in $\strA$ correspond to constraint scopes, and  elements in $\strB$ to values.
	Relations in $\strB$ are constraint relations.

We assume familiarity of the reader with stable models \cite{GL-stable} and Answer Set Programming \cite{DBLP:journals/amai/Niemela99,DBLP:journals/corr/cs-LO-9809032}. The main definitions and examples can also be found, e.g. in \cite{tutorial}. %\footnote{The ASP definitions can be added in an additional page, if required by the PC members.}
}


Least Fixed Point logic FO(LFP) is broadly used in CS and is described in several books.
For a  background on that logic we refer to, e.g. \cite{GraedelEtal:book}.


%Finite model theory (see \cite{Libkin04:book-long}) connects model theory and database research with 
% computational complexity.

\ignore{
Every FO formula $\phi (R, \bar{x})$, where $R$ is a relation symbol of arity $k $ and $\bx $ is a
tuple of $k$ variables, defines, for any structure $\strA$ of appropriate vocabulary, an
operator %$F : P(Ak) ! P(Ak)$ on the class of $k$-ary relations over the universe A of A, namely 
$F : R \mapsto \{ \bar{a} : (\strA,R) \models \phi (R, \bar{a})\}$. If $ \phi$ is positive in $R$,
that is, if every occurrence of $R$ is under an even number of negations, this
operator is monotone in the sense that $R \subseteq R'$ implies $F(R) \subseteq F(R')$. It is
well known that every monotone operator has a least fixed point and a greatest
fixed point, which can be defined as the intersection and union, respectively, of
all fixed points, but which can also be constructed by transfinite induction.
FO(LFP) is defined by adding to the syntax of first order logic the following
fixed point formation rule: If  $\phi(R, \bx)$ is a formula with a relational variable
$R$ occurring only positively and a tuple of first-order variables $\bx$, and if $\bar{t}$ is a
tuple of terms (such that the lengths of $\bx$ and $\bar{t}$ match the arity of $R$), then
$[{\rm lfp} R \bx. \phi ](\bar{t})$ and $[{\rm gfp}R \bx.\phi ](\bar{t})$ are also formulas, binding the occurrences of
the variables $ R $ and $\bx$  in $\phi$.

The semantics of least fixed-point formulas in a structure $\strA$, providing interpretations for all free variables in the formula, 
is the following: $ \strA \models [{\rm lfp} R \bx. \phi ](\bar{t})$ if $\bar{t}^{\strA}$ belongs to the least fixed point 
of the  operator defined by $\phi$  on $\strA$. Similarly, for greatest fixed points.

Note that in formulas $[{\rm lfp} R \bx. \phi ](\bar{t}))$  one may have other free
variables besides $\bx$.
The duality between least and greatest fixed point implies that for any $\phi$,
$[{\rm lfp} R \bx. \phi ](\bar{t})$ and $[{\rm gfp}R \bx.\phi ](\bar{t}) \equiv \neg [{\rm lfp} R \bx. \neg \phi[\neg R / R] ](\bar{t})$.
}

Just as the basic modal logic is a  fragment of first-order logic,  the modal mu-calculus  $ L\mu$ 
 (that includes the well-known temporal logics CTL, CTL$^*$ and LTL) 
 is a fragment of FO(LFP). % (see e.g. \cite{DBLP:conf/aiml/ZaidGJ14} for references).
Moreover, the modal mu-calculus  $L \mu $ is a bisimulation-invariant fragment of monadic second-order logic MSO.
More details on fixed point logics and MSO can be found in  \cite{DBLP:journals/bsl/DawarG02,Libkin04:book-long,GraedelEtal:book}.


\section{Common Reasoning Tasks} 


\subsubsection*{ Three Tasks: Definitions}
For a formula $\phi$ in any logic $\cal L$ with model-theoretic semantics, we can associate the following three tasks
(all three for the same formula), satisfiability (\SAT), model checking (\MC) and model expansion  (\MX).
We now define them for the case where $\phi$ has no free object variables.



\begin{definition}[{\sf Satisfiability (SAT$_\phi$)}]
	\underline{Given:} \\ Formula $\phi$.
	\underline{Compute:} all structures $\strB$
	such that  $\strB\models \phi$. (The decision version is: \underline{Decide:} $\exists \strB$ s.t. $\strB\models \phi$?)
	
\end{definition}

In a modal (temporal) logic setting, this task is usually associated with the non-emptiness problem
for the corresponding automaton.




\begin{definition}[{\sf Model Checking (\MC)}] \label{def:MC}
		\underline{Given:}\\ Formula $\phi$, structure $\strA$ for $vocab(\phi)$.
		\underline{Decide:}  $\strA \models \phi$?
	\end{definition}
There is no search counterpart for this task. Temporal logic model checking is different,
and will be discussed separately.
The following task (introduced in  \cite{MT05-long}) is at the core of this paper.
The decision version of it is of the form ``guess and check'', where the ``check'' part 
is model checking. 
\begin{definition}[{\sf Model Expansion (MX$_\phi^{\sigma}$)}]
	\underline{Given:} \\ Formula  $\phi$ with designated input vocabulary $\sigma\subseteq vocab(\phi)$ and
	$\sigma$-structure $\strA$.
	\underline{Compute:}
	$ \{\strB \ | \ \mbox{ $\strB\models \phi$ and expands}$ \\
		$\sigma$-structure $\strA$ 
	$\mbox{	to $vocab(\phi)$ } \}$.
	(The decision version is: \underline{Decide:} $\exists \strB$ s.t.  $\strB\models \phi$ and expands $\sigma$-structure $\strA$ 
		to $vocab(\phi)$?)
\end{definition}
Vocabulary $\sigma$ can be empty, in which case $\strA$ is just a domain. 
When $\sigma = vocab(\phi)$, we have $\mbox{\sf MX}_\phi^{\sigma} = \mbox{\sf MC}_\phi$.
In general, the domain of the input structure can be infinite. 
%The computational  complexity of the task can be studied in terms of the size of the finite active domain.



 Let $\phi$ be a sentence,
i.e., has no free object variables.
One can look at data, expression or combined complexity, the notions first introduced in \cite{Var82}. 
Data complexity, in terms of the size of the finite active domain, of  \MX lies in-between model checking (full structure is given) and satisfiability (no structure is given).
$$ \mbox{\sf MC}_\phi \leq \mbox{\sf MX}_\phi^{\sigma} \leq \mbox{\sf SAT}_\phi. 
$$
For example, for FO logic, \MC %is boolean query evaluation and 
is non-uniform AC$^0$, \MX captures NP (Fagin's theorem),
and \SAT is undecidable. In all the  tasks except satisfiability,  the (active) domain is always given, which significantly reduces 
the complexity of those tasks.
Examples of the relative complexity of the three tasks for several other logics can be found in \cite{Kolokolova:complexity:LPAR:long}.



\subsubsection*{A more general version of \MX}
We can also define a more general version of the model expansion task 
for formulae $\phi(\bX,\bY)$ with tuples of free relational variables $\bX$ and $\bY$. In this version,   a mapping $v$ of relational variables   to a particular vocabulary is given on the input, or it can be fixed in advance. 
\begin{definition}[{\sf MX$_\phi^{\sigma}$ with free relational variables}]
	\underline{Given:} (1) Formula  $\phi(\bX,\bY)$, where  $\bX$ are the designated relational input variables, $\bY$ are the designated relational output variables, (2) mapping $v: V \mapsto \tau$ of relational variables $V$ to 
	some vocabulary $\tau$, 
	$v(\bX) = \sigma$,  $v(\bY) = \varepsilon$, 
	where  $\sigma, \varepsilon \subseteq vocab(\phi) \subseteq \tau$ and
	(3)	a  $\sigma$-structure $\strA$, where $\strA =(A; \bR) $.\\
	\underline{Compute:}
	$ \{\strB \ | \ \strB\models_v \phi( \bR,  \bR') \mbox{ and $\strB$ expands }  \  \strA  
	\mbox{	to } \tau\}$.
	(The decision version is: \underline{Decide:} $\exists \bR'$ s.t.  $(\strA,\bR)\models_v \phi( \bR,  \bR') $ ?)
\end{definition}
Note that $\strB$ (under vocabulary assignment $v$)  
% is a $\tau$-structure that expands $\strA$,  i.e.,  $\strB =  (\underbrace{A; \bR}_{\fA},  \bR', \dots ) $,
% where $\strB$ interprets $\bX$ by $\bR$, $\bY$ by $\bR'$, all other symbols in $\phi$ in a way that $\strB\models_v \phi( \bR,  \bR')$ holds, and  
interprets symbols in $\tau \setminus vocab(\phi)$ arbitrarily. 
\red{The main advantage of this more general definition is that model expansion turns a formula into a {\em generalized binary relation}.
	We shall use such relations  to construct a reachability relation in a Kripke structure that will allow us to perform
	temporal logic-based reasoning. }




\subsubsection*{Similar Task: Query Evaluation}
In database literature, a task similar to \MX is query evaluation.
We define it for non-boolean queries, i.e., those with free object variables $\by$.
\begin{definition}[{\sf Query Evaluation (\QE)}]\label{def:QE}
	\underline{Given:}\\ (1) Formula  $\phi(\bX,\by)$, where  $\bX$ are the designated relational input variables, $\by$ are the designated object output variables, (2) mapping $v: V \mapsto \tau$ of relational variables $V$ to 
	some vocabulary $\tau$, 
	$v(\bX) = \sigma$,  
	where  $\sigma \subseteq vocab(\phi) \subseteq \tau$ and
	(3)	a  $\sigma$-structure $\strA$, where $\strA =(A; \bR) $.\\
	\underline{Compute:} 	$ \{\bb  \ | \ \mbox{ $\bb$ is a tuple of domain elements, 
	 $|\bb| = |\bx|$,}\\ 	
	\mbox{ and  $\strA\models_v \phi(\bR,\bb )$ } \}$. 
		(The decision version is: \underline{Decide:} $\exists \bb$ s.t.  $\strA \models_v \phi( \bR,  \bb) $ ?)
\end{definition}


\blue{While model expansion can be viewed as a non-deterministic action (with potentially an exponential number of structures-outcomes, in terms of the size of the input domain), query evaluation 
is always a deterministic action. }

\ignore{
\subsubsection*{Related Tasks: Model Checking for Formulae with Free Object or Free Set Variables}

Definition \ref{def:MC} could be reformulated as: 


\begin{definition}[ \hspace{-3mm} \MCx, free object variables]
	\underline{Given:} $\psi(\bx)$,  tuple of domain elements $\ba$, and 	$\sigma$-structure $\strA$, where $\sigma= vocab(\psi)$
	(as in Definition \ref{def:QE}).
	\underline{Decide:}  $\strA \models \psi[\ba]$?
\end{definition}





For finite structures, query evaluation (for queries with free object variables) is reducible to model checking, but not necessarily in general.  

For formulae with free relational variables (no free object variables), Definition \ref{def:MC} could be reformulated as 




\begin{definition}[\MCX, free set variables] {\ }\\
\underline{Given:} Formula  $\phi(\bar{X})$ with free relational variables  $\bar{X}$, each 
	ranging over domain elements, tuple of relations $\bar{R}$, and
	$\sigma$-structure $\strA$, where $\sigma= vocab(\phi)$.
	\underline{Decide:}  $\strA \models \phi[\R]$? \blue{notation does not work in the proposition}
\end{definition}

}



%The decision version of \MX  is connected to \MCX, but has a  ``guess'' part in addition.





%This version of model checking is NOT similar to temporal model checking. The state we check is the database given on the input, 
%not the expansion (output part).




\ignore{
\subsubsection*{Model Expansion versus Query Evaluation}

As a side remark, note that we could have defined a more general version of QE,
	where the variables $\bx$ would allowed to be SO. Then MX would be a particular case of this extended notion of query evaluation. 
 However, that would  contradict the definition of a query e.g. in Immerman's book \cite{Immerman-book} (see page 17) as a mapping from 
 structures in one vocabulary to structures in another vocabulary that is polynomially bounded. The size of the set 
 $\mbox{\MX}(\strA)$  {\tt NOTATION }??????????? can be
 exponential in the size of $\strA$.
}
For {\em the same logic}, these two tasks, \MX and \QE, (as we defined them)  have very different computational complexity, --
e.g., for FO, query evaluation is in AC$^0$, model expansion is NP-complete. %For this reason, we prefer to treat them separately.
%Model expansion corresponds to a non-deterministic action in the dynamic setting, while QE is deterministic.
There is an  analogy between sets of tuples generated by  \QE {\ } and sets of structures in \MX. {\tt This analogy will be revisited later in this paper. ??????}
%The same analogy can be seen in  Immerman's results in descriptive complexity for extensions of SO logic \cite{Immerman:capturing}.




\subsubsection*{The  Tasks (\MC, \MX, \SAT, \QE) in Applications}

In database research, \QE  {\  } has already been  studied extensively, e.g.   for FO logic (Codd's relational algebra) 
and its fragments (e.g. for  conjunctive queries), as well as for DATALOG and its variants.
\SAT has demonstrated its practical importance mostly for propositional logic, a logic of a very low expressive power.
Indeed,  the success in SAT solving (achieved both by smart algorithms and an exponential growth in hardware capabilities)
is one of the most remarkable achievements of logic in CS. Due to this success, the complexity class NP
is often called ``the new tractable''. However beyond the propositional case, the great majority of logics that are interesting and useful in Computer Science 
are undecidable. For instance, first-order logic is undecidable even in the finite (by the Trakhtenbrot's theorem).
While decidability continues to be discussed in many papers, the importance of this task for practical logics
is greatly overrated. On the other hand,  {\em unlike satisfiability, model expansion (along with query evaluation) for expressive logics 
	has much better computational properties} \cite{Kolokolova:complexity:LPAR:long}. This   task  has not yet been sufficiently studied,
yet it is very common in practise.



Just as the query evaluation problem is prevalent in database research, model expansion is very common in the general area of constraint solving.
Most constraint solving paradigms solve \MX as the main task, e.g. \red{ REPLACE WITH CSP AND DB EXAMPLES LOGICBLOX in AI planning, scheduling,
logistics, supply chain management, etc.
Java programs, if they are of input-output type, can be viewed as 
model expansion tasks, regardless of what they do internally.} Most combinatorial problems are of that form, many software programs (e.g., web services) and hardware devices (e.g., circuits) are of that form.  The Logistics Service Provider in Example  \ref{ex:LSP} has, e.g., customer requests
as an input, and routes and packing solutions as  outputs.
In Example \ref{ex:HC-2Col}, one can 
have e.g. edges of a graph on the input 
to formula  (\ref{3-Col-HC}), and colours on the output.  ASP systems, e.g., Clasp \cite{clasp} mostly solve model expansion, 
and so do CP languages such as Essence \cite{Essence}, as shown in \cite{MT-essence-journal:2008}. Problems solved in ASP competitions are mostly 
in model expansion form.
CSP in the traditional AI form (respectively, in the homomorphism form) is representable by model expansion where mappings to domain elements (respectively, homomorphism functions) are expansion functions. Several examples are given in the \blue{Appendix ?????????}.
\footnote{\red{Talking about these systems answering second-order queries 
		would be mathematically correct, but impractical since their languages are often very far from classical logic, and may be even imperative.???????????}}




{\em Model expansion for an expressive logic  and satisfiability for a corresponding (and much less expressive) logic are connected in the same way as Fagin and Cook's theorems are connected (see, e.g. page ??? of \cite{Libkin04:book-long}), through a step that in practical systems is called {\em grounding}, that amounts to instantiating variables with constants that correspond to the domain of the instance structure. }
For example, this step is implemented in ASP systems e.g. Clasp \cite{clasp}. \blue{Enfragmo} \footnote{In the ASP literature, inputs are given as sets of ground atoms,
	and the semantics is discussed in terms of Herbrand structures, which obscures the separation of problem instances (structures, databases, a semantical notion here) from problem descriptions (axiomatizations of combinatorial problems).} 


===============

We shall view $\phi$ in \MX as axiomatizing a class of structures, that we call a {\em module}, where the free SO
	variables are \red{ not always fixed in advance.}
This task adds information flow to \red{the algebra}, which turns it into a modal temporal logic similar to 
the Propositional Dynamic Logic (PDL), as we explain below.





\ignore{
Almost all  non-trivial commercial software systems use libraries of reusable components.
Component-based engineering is also widely used in VLSI circuit design, supported by a large number
of libraries.
The theory of combining conventional imperative programs and circuits is relatively well-developed. 
However, in knowledge-intensive computing, characterized by using so-called declarative programming, 
research on {\em programming from  reusable components} is not very developed\footnote{Related work that is most relevant is discussed at the end of the paper.}. 
%{\tt explain solbing combinatorially hard problems in industry. As Michel and van Henderic noted...} 
 It would  be very desirable to be able to take a program written in Answer Set Programming (ASP), combine it (say, as a non-deterministic choice)  with a specification of a Constraint Satisfaction Problem (CSP), and 
then, sequentially, with an Integer Linear  Program (ILP), and send  feedback as an input to one of the first two programs. Such a programming method,
from existing components, possibly found on the web, would be extremely useful.
The main challenge however
is that the programs may be written in different languages (even legacy 
languages), and rely on different solving technologies.

% for non-programmers who find existing components on the web.
%}


%\noindent {\bf Integration} 



Recently, there has been a lot of work on technology integration. Examples include but are not limited to 
\cite{DBLP:journals/amai/MellarkodGZ08,DBLP:conf/lpnmr/BalducciniLS13,DBLP:conf/cpaior/0001KMO14,ASP-CP-combination,Picat}. %We do not attempt  a comprehensive survey, but we highlight some important issues.
Combined solving is perhaps most developed in the SMT community, where theory propagations are tightly interleaved with satisfiability solving
\cite{DBLP:journals/jacm/NieuwenhuisOT06,SMT}.
 Declarative and imperative types of programming sometimes have to be combined for best results.



Solving methods often rely on  {\em decomposition} which are also studied in knowledge representation. 
A method for large knowledge base decompositions is developed by E. Amir and  S. McIlraith   \cite{DBLP:journals/ai/AmirM05}. Tree decompositions
are used to tame complexity in the work by  S. Woltran and colleagues \cite{DBLP:conf/jelia/AbseherBCDHW14,CharwatWoltran:LPNMR:2015}. 
Several similar notions of  {\em tightening - relaxation},  {\em abstraction - refinement}, as well as  several notions of 
{\em equivalence} are used in 
constraint solving and hierarchical program development.  

%Assistant tools, e.g. for hierarchical development 
%and domain-specific  control are needed.  ...... control that can later be refined in a declarative or imperative way.	  

%Bisimulation and other notions of equivalence (e.g. trace-equivalence) are used.  

%{\tt operations ... control (it did not become completely clear to me what 
%	you mean by these terms in this context)}




For efficient solving, {\em special propagators} are identified and either implemented separately or integrated tightly into the main 
reasoning mechanism.
For example, acyclicity \cite{DBLP:conf/ecai/GebserJR14} is added to SAT and ASP as a special propagator. 
BDDs are also used as special (and more powerful) propagators in hybrid constraint solving 
\cite{DBLP:journals/jair/GangeSL10}.
Experts can identify special sub-problems, which might still be combinatorially hard, but  the solutions of which can help to solve the main 
problem. 
It is desirable to specify domain-specific  propagators declaratively. A method for writing such specifications 
is proposed in our recent work \cite{TT:LaSh:2014}. 

% usually produced with the help of experts who understand the problem
% in consideration in-depth. 

%It is inevitable that, in solving combinatorial constraint and optimization problems,   the knowledge of 
%domain expert plays an important role and is incorporated into solving strategies.


% usually produced with the help of experts who understand the problem
% in consideration in-depth. 




Various kinds {\em of meta-reasoning} are used on top of knowledge-intensive methods.
Meta-reasoning (high-level control) is used, for example, in {\sf dlvhex}, a nonmonotonic logic programming system aiming at the integration
of external computation sources and higher-order atoms \cite{dlvhex}. 
Sophisticated control is used in \cite{DBLP:journals/jair/CatDBS15}, where the authors
%(B. de Cat,
%M. Denecker,
%M. Bruynooghe and
%P. Stuckey)
 develop a method for lazy model
expansion, where the grounding is generated lazily (on-the-fly) during search.
%The approach works by associating justifications to the non-ground parts of the theory.
%B. Bogaerts,
%J. Jansen, B. De Cat, G. Janssens, M. Bruynooghe and M. Denecker 
The authors  of  \cite{bootstrapping-LASH} use bootstrapping for the IDP system, where inference engine itself is used to tackle some tasks solved inside a declarative  system declaratively.





%{\tt The knowledge of domain experts is usually used to perform those decompositions, 
%	and to identify special-purpose  propagators.}


%Their knowledge is  programmed  in special shells built on top of, and in order to control declarative modules \cite{shells}. Also,in CP?


 
 
 However, practical constraint solving remains a complex task.
 K. Francis noted, in \cite{Francis:ModRef:2014}:
``The results of the 2013 International Lightning Model and Solve competition
served as a reminder that our tools are too hard to use. The winners solved the
problems by hand, suggesting that creating an effective model was more time
consuming (or daunting) than solving the problems.'' 


%{\tt integration of subprograms is controllable from the procedural side}  \cite{Clingo-ASP-Control}


  
 


Several research questions still need to be answered to bring solving and development technologies to the next level.

\begin{enumerate}

\item  The technologies are diverse, some use declarative representations, some are purely imperative. 
What is common in all those advanced technologies, what would be a basis for integration?
	What are the units we combine, decompose into? 
	
\item	How can we combine those units? 
	The language of combinations should be both expressive and feasible computationally.


\item  What is the notion of a solution, how can such modular systems  be solved? 

\item  What is (are) reasonable notion(s) of equivalence, modular system containment? 

\end{enumerate} 

Our main goal is to provide a mathematical basis for combined constraint solving, and for specifying high-level control of such solving. %{\tt add from LPNMR submission}

%{\tt rapid prototyping of solving complex problems, hierarchical development, module reuse}
	
 We believe that integration of technologies, from separate communities {\em cannot be done on the basis of  one language}. 
Communities that  develop technologies are attached to their languages. Experts usually get training (often during their PhD study) in one technology, and 
tend to keep applying it. It would be a utopia to assume that everyone would eventually switch to using a common representation language. 
It is also impractical to assume that axiomatization of each module would be translated to one language for solving. 
In such a translation, language-solver-specific  efficiency adjustments in axiomatizations would be lost.
Thus, a  language-independent way of integration is needed. Since \cite{TT:FROCOS:2011-long} we have been arguing that 
model theory is a good basis for integration in a language-independent way.  



In this paper, we continue the line of research we started in  \cite{TT:FROCOS:2011-long} where 
Modular Systems  were introduced. They were further developed in \cite{Shahab-thesis,Newman-thesis,TWT:WLP-INAP:2012,TT:NMR:2014,TT:KR:2014,MT:LPNMR:2015,ET:IJCAI:2015,TT:HR:2015}.
{\em The main conceptual shift proposed in those works was to take model-theoretic approach seriously}.   
Due to the model-theoretic view, the formalism is language-independent, and combines modules  specified in {\em arbitrary 
	languages}.









 
 



 A formalism for combining such programs should allow for arbitrary languages, and, at the same time, should lay foundations 
 for solving combined systems,  employing the solving power of solvers for  languages used in the system.
It should provide {\em heterogeneity in the syntax}, 
{\em homogeneity in the semantics}. Heterogeneity in the syntax is important because modules can be represented 
in different languages. Homogeneity in the semantics is crucial for developing efficient solving algorithms.
The first question is  what a {\em module} is. In addition,
 a {\em small but expressive} set of operations for combining modules  is needed. 
 %It should allow one to express at least sequential and parallel composition,  synchronization, non-deterministic choice and projection. 
The formalism  should have {\em controlled expressiveness.}
On one hand, it should have {\em enough  expressive power} to be able to produce interesting and useful combinations of modules,
provide guarantees to be able to represent any problem, if its complexity is within the power of the language.
On the other hand, the formalism should be {\em efficiently implementable}.
Note that there is a tension between these two requirements. An increase in expressive power 
comes at the expense of efficiency.  
%The algebra we  describe strikes a good balance between complexity and efficiency.      
Finally, the formalism should contain a small number of operations, but sufficient  for specifying high-level control.



In this paper, we define the notion of a module, which is language-independent, and describe an algebra for combining such modules, and consider its version with information propagation. We draw parallels with Codd's relational algebra, and 
process algebras originating from the work of Hoare and Milner. 
%We talk about decompositions by means of our algebra. Decompositions are used to come up with special propagators and identify high-level execution control structure.
We discuss meta-solving, 
where the main solver is viewed as a  ``master'' communicating with ``slaves'',
individual modules that may have their own solvers associated with the  language of the module (e.g., CSP, ASP modules). We argue, from the complexity-theoretic 
perspective, that such meta-solving is possible, for an interesting fragment, with the current technology for solving problems in the complexity class NP.


%{\tt Such methods of solving can be applied to arbitrary theory combinations in SMT and combinatorial optimization, along the 
%	lines of \cite{Michel} }


Several notions of inclusion (abstraction-refinement) and equivalence are possible for our algebra. 
We discuss two, one has more set-theoretic flavour, and the other is more behaviour-based. 




The paper contains two main parts. The first part, presented in Section \ref{sec:Algebra}, describes the general version of our algebra of modular
systems. The second part, presented in Section \ref{sec:Algebra-Inf-Flow}, defines a directional variant of the algebra,
where the information flow is specified. 


%{\tt without going into details, we can mention that the two parts (even though they are higher-order) are connected 
%	as FO(LFP) and the modal fragment $L_\mu$.}

}
